Co-Designed Architectures for Modular Superconducting Quantum Computers

Noisy, Intermediate Scale Quantum (NISQ) computers have reached the point where they can show the potential for quantum advantage over classical computing. Unfortunately, NISQ machines introduce sufficient noise that even for moderate size quantum circuits the results can be unreliable. We propose a co-designed superconducting quantum computer using a Superconducting Nonlinear Asymmetric Inductive eLement (SNAIL) modulator. The SNAIL modulator is designed by considering both the ideal fundamental qubit gate operation while maximizing the qubit coupling capabilities. First, the SNAIL natively implements $\sqrt[n]{\texttt{iSWAP}}$ gates realized through proportionally scaled pulse lengths. This naturally includes $\sqrt{\texttt{iSWAP}}$, which provides an advantage over $\texttt{CNOT}$ as a basis gate. Second, the SNAIL enables high-degree couplings that allow rich and highly parallel qubit connection topologies without suffering from frequency crowding. Building on our previously demonstrated SNAIL-based quantum state router we propose a quantum 4-ary tree and a hypercube inspired corral built from interconnected quantum modules. We compare their advantage in data movement based on necessary \texttt{SWAP} gates to the traditional lattice and heavy-hex lattice used in latest commercial quantum computers. We demonstrate the co-design advantage of our SNAIL-based machine with $\sqrt{\texttt{iSWAP}}$ basis gates and rich topologies against $\texttt{CNOT}$/heavy-hex and $\texttt{FSIM}$/lattice for 16-20 qubit and extrapolated designs circa 80 qubit architectures. We compare total circuit time and total gate count to understand fidelity for systems dominated by decoherence and control imperfections, respectively. Finally, we provide a gate duration sensitivity study on further decreasing the SNAIL pulse length to realize $\sqrt[n]{\texttt{iSWAP}}$ qubit systems to reduce decoherence times.

==> extra-stuff.tex <==
\subsubsection{Virtual-Z Decomposition}
To this point the cost of 1Q gates has been considered negligible. This is only true if it is possible to calibrate a finite set of 1Q gates and decompose an arbitrary 1Q gate into a few basis gates. In practice, arbitrary 1Q gates must be constructed using only a discrete set of calibrated 1Q gates. The Solovay-Kitaev theorem provides a route to follow, using a finite set of gates consisting of the Hadamard gate (\texttt{H}) which flips a qubit's $X-$ and $Z-$polarization components, and 1Q Z-rotations by $\pi/2$ and $\pi/4$, the so-called \texttt{S} and \texttt{T} gates~\cite{nielsen2002quantum}. In most experimental implementations, however, the native gates are continuous rotations about the qubit $x-$ and $y-$axes via in-phase and quadrature driving of the qubit's energy transition, in direct analog to the controls present for spins in nuclear  magnetic resonance or electron spin resonance\cite{N&C}. \akj{NMR and ESR?  I think some explanation may be missing here} In this implementation there is no physically applied $z-$axis rotation gate to implement \texttt{S} and \texttt{T} gates; these correspond instead to an instantaneous phase shift in the classical control electronics. Since we can very finely control and stabilize this drive phase (indeed precise 1Q gate controls require exactly this), we can extend the idea to a continuous, virtual (zero duration hardware) Z rotation as previously demonstrated~\cite{asdfa}.  

\begin{equation}
    \label{virtualz}
    U(\theta, \phi, \lambda) = Z_{\phi-\pi/2} \cdot X_{\pi/2} \cdot Z_{\pi - \theta} \cdot X_{\pi/2} \cdot Z_{\lambda-\pi/2}
\end{equation}

Consequently, calibrating only a single hardware gate, for example $\sqrt{X}$, in conjunction with virtual-Z gates retains the power to express the continuous set of arbitrary 1Q gates stated by Eq.~\ref{virtualz}.  Thus, an arbitrary 1Q gates costs at most 2 single qubit gates to implement; this, together with the short duration/high fidelity of single qubit rotations motivates our convention throughout this manuscript that 1Q gates have negligible duration and cost.

As discussed, the remaining non-virtual 2Q hardware gates are analog pulses which actuate a time-dependent coupling between two or more qubits. Practically, this qubit-qubit coupling arises from a physical connection between them.  These can take simple forms, from a simple capacitive coupling to a more elaborate nonlinear circuit.  We will refer to them generally as \textit{modulators}, which may target pairs of qubits via layout geometry, unique frequencies or frequency differences, and which, together with applied control signals, govern the fundamental gate operation implemented in the quantum computer. In the next section the coupling neighborhoods, formed from the combination of modulator and physical connections, are described in more detail.  



The minimum requirements for a quantum computer are given by the DiVincenzo criteria \cite{divincenzo2000physical}: (1) a scalable method for creating quantum two-level sytems, or quantum bits (qubits), (2) the ability to initialize the state of the qubits reproducibly, (3) long coherence times for the qubits, (4) a `universal' set of quantum gates, and (5) the ability to read out the state of each qubit with high fidelity.




\subsubsection{Cartan's KAK Decomposition} 
%https://arxiv.org/pdf/quant-ph/0209120.pdf
%https://arxiv.org/abs/quant-ph/0507171
Unitary operators obey special rules of periodicity and commutation that allows for conveying relationships between 2Q gates geometrically using a triangular tetrahedron known as the ``Weyl chamber''~\cite{zhang2003geometric}. Unitaries that can be made equivalent with the addition of 1Q gates are called locally invariant, and occupy the same coordinates of the Weyl chamber. Additionally, as the canonical gate shown in Eq.~\ref{canonicalgate} is parameterized by coordinates of the Weyl chamber, with the proper 1Q gates it can express any 2Q unitary.
\begin{equation}
    \label{canonicalgate}
    \texttt{CAN}(t_x,t_y,t_z) = \exp{(-i \frac{\pi}{2}(t_x X \otimes X + t_y Y \otimes Y + t_z Z \otimes Z))}
\end{equation}

The decomposition strategy, known as the KAK decomposition is outlined as follows. First, diagonalize the target arbitrary unitary in the canonical gate basis and extract Weyl chamber coordinates from the eigenvalues. In other words, find the coordinate parameters of the canonical gate as in Eq.~\ref{canonical gate}. Next, use the desired native 2Q basis gate interleaved with 1Q gates to sufficiently span regions of the Weyl chamber. Finally, solve for the interleaved 1Q gate parameters to have rebuilt the target unitary~\cite{tucci2005introduction}. 

Depending on the 2Q basis gate and the region of the Weyl chamber the canonical gate occupies determines how many times the 2Q basis gate must be interleaved with 1Q gates. Prior work has derived a set of Weyl chamber spanning rules for $\sqisw$ such that for all 2Q unitaries, decomposition requires at most three $\sqisw$ gates~\cite{huang2021towards}, as in Figure~\ref{sqiswap-decomp}. 

%\akj{Move the following to experimental setup}  The explicit outlining of this procedure allowed us to implement the $\sqisw$ decomposition in our transpiler's basis translation.
%\usepackage[braket, qm]{qcircuit}
\begin{equation}
\label{canonical gate}
\scalebox{0.95}{
\Qcircuit @C=1.0em @R=0.4em @!R {
	 	\multigate{2}{\mathrm{U}} & & & \gate{\mathrm{U_1}} &
	 	\multigate{2}{\mathrm{\texttt{CAN}(t_x,t_y,t_z)}} & \gate{\mathrm{U_3}} & \qw
	 	\\
	 	& \push{\rule{0em}{0em}=\rule{0em}{0em}}
	 	\\
	 	\ghost{\mathrm{U}} & & & \gate{\mathrm{U_2}} &
	 	\ghost{\mathrm{\texttt{CAN}(t_x,t_y,t_z)}} & \gate{\mathrm{U_4}} &\qw
	 	\\
}}
\end{equation}

% \mjh{need to be clear: find canonical gate to give coordinates. Separately, works such as blah show templates like equation 6 and show which regions of Weyl chamber you can do w/ 1,2,3 applications, and allow you to take canonical gate to cost, and with some work to fine 1Q gates to actual decomposition}

Intuitively, this mimics the example strategy as before, making a substitution for every $\cnot$ with 2 $\sqisw$s. However, unlike for $\cnot$ as an intermediary translation step, a single use of $\texttt{CAN}$ is itself sufficient for generating arbitrary 2Q unitaries and thus is exactly as efficient as translating directly to $\sqisw{}$. 

\begin{equation}
\label{sqiswap-decomp}
\scalebox{0.90}{
    \Qcircuit @C=0.4em @R=0.4em @!R {
	 	\multigate{2}{\mathrm{U}} & & & \gate{\mathrm{U_1}} & \multigate{2}{\mathrm{\sqisw}} & \gate{\mathrm{U_3}} &
	 	\multigate{2}{\mathrm{\sqisw}} & \gate{\mathrm{U_5}} &
	 	\multigate{2}{\mathrm{\sqisw}} & \gate{\mathrm{U_7}} & \qw
	 	\\
	 	& \push{\rule{0em}{0em}=\rule{0em}{0em}}
	 	\\
	 	\ghost{\mathrm{U}} & & & \gate{\mathrm{U_2}} & \ghost{\mathrm{\sqisw}} & \gate{\mathrm{U_4}} &
	 	\ghost{\mathrm{\sqisw}} & \gate{\mathrm{U_6}} &
	 	\ghost{\mathrm{\sqisw}} & \gate{\mathrm{U_8}} &\qw
	 	\\
	 }}
\end{equation}

Furthermore, the physical controls (\textit{i.e.,} pulses) that create gates are typically analog and continuous.  So, theoretically it is possible to decompose 2Q unitaries into $\sqisw[n]$ using very short pulses finely interleaved with 1Q unitaries which we explore in Section~\ref{section:approxdecomp}.  However, if we limit ourselves to $n \in \{1,2\}$, then all 2Q gates follow the form of  Eq.~\ref{sqiswap-decomp} such that all 2Q gates can be decomposed in one, two, or three  $\isw$ family gates plus necessary 1Q gates.


%this is getting moved into normalization argument
\subsubsection{Comparison between \texorpdfstring{$\cnot$}{CNOT} and \texorpdfstring{$\sqisw$}{SQiSW}} %\mjh{note to self: pick up here tomorrow and make this a less math intense story.  Idea: are they just as good, how do we assign an advantage to one over the other:  (0) lets limit ourselves to two gates (not further fractioning for now) so an arbitarry U requries 0-3 2Q gates.   (a) either you have an 'average' advantage because better at making gates with on average fewer gate or (b) you have an algorithm that makes one kind of gate all the time/way more often.  Examples: QFT loves fractional ctrl-Z, GHZ all CNOTs, or... in machine w/ out all-to-all SWAPs can be most commmon...}

% \akj{maybe some of this can move to motivation}
% \emc{I've tried to find a gate that takes only 2 sqiswap gates compared to 3 CNOT gates because I know many must exist but I'm having a hard time reverse engineering one for sake of demonstration - not sure if this would be important to have here or not}. 
% \akj{maybe for illustration, what's more important is to show the critical properties that Alibaba is showing, not just copy their conclusions...}
% \akj{remove this quote and show the math if its useful}. \textit{Moreover, we prove that 79\% of two-qubit gates (under the Haar measure) can be generated using only two uses of the SQiSW gate. As a comparison, only a zero-measure set of two-qubit gates can be generated using two uses of common two-qubit gates such as CPHASE family gates, SWAP family gates or the iSWAP gate. Furthermore, we prove that in the task of generating certain W-like states, we need strictly less SQiSW gates compared to iSWAP or CNOT gates.\akj{this seems like the answer to above} These results suggest that while SQiSW is the square root of iSWAP, its information processing capabilities can rival and even surpass that of iSWAP and CNOT in multiple meaningful aspects}~\cite{huang2021towards}
% \akj{what percentage of two-quibit gates can be constructed from \cnot{}?}

%idea behind haar measure- if you just take equal distributions of the parameters of an arbitrary unitary that doesn't equate to a uniform distribution. Think bloch sphere- there are more states centered around the equator than the poles so a naive distribution would be favoring the poles if it sampled states from an even distribution of latitudes. 

% After developing methods for translation into either the $\cnot$ or $\sqisw$ basis, it is appropriate to question which basis set is generally more useful. As previously mentioned, the best choice of a basis gate depends on what is most natural for a particular hardware to implement. Not only do superconducting qubits conveniently produce $\isw$-family gates, but according to a Weyl chamber metric of effective target size, $\sqisw$ has a comparatively larger invariant volume subject to small perturbation, thus being easier to physically realize \cite{huang2021towards}. 

Given both $\cnot$ and $\sqisw$ are universal and require at most three instances to implement an arbitrary 2Q gate, they seem at least pseudo-equivalent.  However, they do not always require the same number of instances to translate a given non-native gate. For example, to implement a $\czgate$ gate requires only a single usage of $\cnot$ as they are locally invariant to one another, whereas 2 $\sqisw$ gates are needed. Thus, for an algorithm that makes heavy use of $\czgate$ gates, $\cnot$ would be a more efficient native gate.  For another important quantum algorithm, the Quantum Fourier Transform (QFT), the un-translated gates consist exclusively of CPhase-family gates~\akj{is this too out of the blue?}, which generally require two $\cnot$ or two $\sqisw$ to translate.  In NISQ machines, as we will show below, data movement via $\sw$ gates can dominate many algorithms; $\sw$ requires three uses of either $\cnot$ and $\sqisw$. 

While in this sparse sampling, $\cnot$ appears to have a slight edge over $\sqisw{}$, in general, for a randomly distributed selection of 2Q gates, the $\sqisw$ requires only 2 uses far more often than the $\cnot$~\cite{huang2021towards}. 

Intuitively, the percent of gates that can be generated relates to the volume occupied inside the Weyl chamber. Two uses of $\sqisw$ forms a tetrahedron, whereas two uses of $\cnot$ lie merely along a plane. This suggests that for random quantum algorithms, or algorithms using a diverse gate set, $\sqisw$ should be more efficient.
% Thus, another useful information-theoretic measure is of what percent of 2Q gates can be generated from only two uses of each gate. Whereas 79\% of 2Q gates can be generated from $\sqiswap$ under the Haar measure, which yields a uniform distribution to sample 2Q gates from, only a "zero-measure set" can be made from two uses of $\cnot$  


% Finally, it is known that the $\sqisw$ gate is the smallest fraction of $\isw$ that remains as a perfect entangler \cite{huang2021towards}. All of which is good evidence of the ease and efficiency of $\sqisw$ as a basis gate. However, we go on to explore smaller fractional exponents of $\isw$ in section \ref{section:approxdecomp}.

%https://arxiv.org/pdf/quant-ph/0312193.pdf
%this paper is stating that although the B gate is even better than sqiswap information processing capabilities - it is too hard to physically realize. So our point is that sqiswap is best compromise 
% "Since the B gate is optimal in
% constructing a quantum circuit, this suggests that one
% might always prefer to implement B as the elementary
% two-qubit gate for any given physical system. However,
% the ease and efficiency of constructing the elementary
% gates for quantum computation from an available Hamiltonian is also a critical issue for realization of quantum
% circuits [17, 18, 19]. Optimally efficient construction of
% quantum operations is realized by the quantum circuit
% which contains a minimal number of single- and twoqubit gates, where each gate is itself also implemented
% with a minimal application time."

==> revision_notes.tex <==
\section{Appendix}
List of changes/additions made for revision in the order that they appear.
\begin{enumerate}
    \setcounter{enumi}{-1}
    \item Abstract
        \begin{enumerate}
            \item Rewritten to be less vague and enumerate work done in the revised paper
        \end{enumerate}
    \item Introduction
    \begin{enumerate}
        \item Figure for quantum computing stack, annotating the region where we do co-design
        \item Paragraph about what is co-design 
        \item Justification for extrapolating small experimental work to large theoretical scale via co-design, 
        \item Concluding remark that links paper results back to co-design.
    \end{enumerate}
    \item Background and Preliminaries
    \begin{enumerate}
        \item Short clarification of KAK decomp. 
        \item Justification for stating its more efficient to decompose directly into basis gate.
        \item Reword common qubit topologies to make clear we are using hex-lattice because it was in iteration of IBM designs. 
        \item Emphasize text in red for question what are the advantages of the hypercube.
        \item Concluding statement which clarifies what is previous work and new novel work. 
    \end{enumerate}
    \item Motivation
    \begin{enumerate}
        \item Emphasize text in red for the merit of our evaluation metrics using gate counts rather than fidelities for reliability. 
        \item Removed the 16-qubit test on basic topologies which conveyed that higher average topology connectivity degree is advantageous but uniquely insightful with the same plot kept in just on the larger topologies.
        \item Combine Observation 2 and 3 per the removal of the 16-qubit test.
    \end{enumerate}
    \item SNAIL Parametric Modulator
    \begin{enumerate}
        \item New intro defining Hamiltonian in relation to unitary gates
        \item Reordered paragraphs so concepts flow more logically, removed some unnecessary physics descriptions
        \item Add equation that shows how SNAIL Hamiltonian relates to \isfam
        \item A statement about why 3rd order terms are desirable because pump power trades with shorter gate duration
        \item Emphasize text in red to clarify there is not a bottleneck on the SNAIL because gates can be done in parallel
        \item Comment clarifying what is previous work
        \item Description of the parametric driven exchange figure given more context, how it relates to gates and fidelity
        \item Paragraph explaining SNAIL fidelity limits and normalizing engineering efforts
        \item Comment clarifying what is previous/new work
        \item Figure with in-text description on how 84-qubit Trees are built
        \item Description of what SNAIL module configurations are possible
        \item Description of the module connections to build corral with comments about its feasibility
    \end{enumerate}
    \item Experimental Setup
    \begin{enumerate}
        \item Comment clarifying we don't build a larger corral in this paper instead are using the hypercube for 84 size.
        \item Rewrote experiment setup description to make more clear how we use Qiskit
        \item Figure of transpilation flow for clarity of data collection process
        \item Clarification of why choose which algorithms to include in our benchmark
        \item Explicit description of the parameters we collect
        \item Restate a better evaluation metric is gate counts rather than fidelities
    \end{enumerate}
    \item Result
    \begin{enumerate}
        \item Figure 13 has Corral data line that was missing from original version
        \item Comment that the Corral topology consistently outperforming
        \item Rewriting for clarity statement about hypercube stability and noisy-data from approximation algorithms
        \item Approximation Decomp section relabeled as Pulse Duration Sensitivity Study
        \item Reorganized and expand explanation of analytical approximation decomposition methods
        \item Explicitly defining equations for hilbert-schmidt inner product,decomposition fidelity and best total fidelity.
        \item Data Figures now include both x-axis using gate count and pulse duration
        \item Data Figure for total fidelity switched x-axis and data lines, now the x-axis is F(iSwap) and each line is a basis gate
        \item Data Figures now include 6th and 7th -root iSwap.
    \end{enumerate}
\end{enumerate}
